CoinMagic: A Differential Privacy Framework for Ring Signature Schemes

By allowing users to obscure their transactions via including "mixins" (chaff coins), ring signature schemes have been widely used to protect a sender's identity of a transaction in privacy-preserving blockchain systems, like Monero and Bytecoin. However, recent works point out that the existing ring signature scheme is vulnerable to the "chain-reaction" analysis (i.e., the spent coin in a given ring signature can be deduced through elimination). Especially, when the diversity of mixins is low, the spent coin will have a high risk to be detected. To overcome the weakness, the ring signature should be consisted of a set of mixins with high diversity and produce observations having "similar" distributions for any two coins. In this paper, we propose a notion, namely $\epsilon$-coin-indistinguishability ($\epsilon$-CI), to formally define the "similar" distribution guaranteed through a differential privacy scheme. Then, we formally define the CI-aware mixins selection problem with disjoint-superset constraint (CIA-MS-DS), which aims to find a mixin set that has maximal diversity and satisfies the constraints of $\epsilon$-CI and the budget. In CIA-MS-DS, each ring signature is either disjoint with or the superset of its preceding ring signatures. We prove that CIA-MS-DS is NP-hard and thus intractable. To solve the CIA-MS-DS problem, we propose two approximation algorithms, namely the Progressive Algorithm and the Game Theoretic Algorithm, with theoretic guarantees. Through extensive experiments on both real data sets and synthetic data sets, we demonstrate the efficiency and the effectiveness of our approaches.

==> problemvariant.tex <==
\section{A Practical Variant of CIA-MS}
\label{sec:variant}
In this section, we introduce a practical variant of CIA-MS, namely the CIA-MS problem with disjoint-superset constraint (CIA-MS-DS). We first define the CIA-MS-DS problem. Then we formally introduce the notions used in the CIA-MS-DS problem definition and its significant properties.

\subsection{The CI-aware Mixins Selection with Disjoint-superset Constraint Problem}
In the related ring signature set $\mathbb{R}$, a ring signature may be the superset of some its previous ring signatures and none of its subsequent ring signatures is its superset. We name such a ring signature as a \textbf{super ring signature}. In this subsection, we formally define the CIA-MS-DS problem, which is a special variant of the CI-MS problem, where for any two super ring signatures, $srs$ and $srs'$, in the related ring signature set $\mathbb{R}$, if $srs \cap srs' = \emptyset$. We name such a related ring signature set as a \textbf{disjoint-superset ring signature set}. Besides, the new ring signature $r$ should satisfy that for any ring signature $r'$ in the ring signature set $\mathbb{R}$, if $r \cap r' \neq \emptyset$, $r' \subset r$. Thus, we can get a set, $\mathbb{M}$, of modules, where each \textbf{module} $m_i$ is a coin that has not been contained in any ring signature in $\mathbb{R}$ or is a super ring signature. The new ring signature is composed of some modules in $\mathbb{M}$.

\begin{definition}
	(The \underline{CI}-\underline{a}ware \underline{m}ixins \underline{s}election with \underline{d}isjoint-\underline{s}uperset constraint (CIA-MS-DS) problem) Given a module set $\mathbb{M}$, the coin $c_\tau$ that will be spent, a required $\epsilon$, and a budget $B$, a user wants to pick up a set of mixins, combining $c_\tau$, to generate the new ring signature $r_{m+1}$, such that its diversity $dive_{r_{m+1}} = |\{t_i | c_i \in r_{m+1}\}|$ is maximized and the following constraints are satisfied:
	\begin{itemize}[leftmargin=*]
		\item \textbf{SRS constraint} $r_{m+1}$ is composed of some modules in $\mathbb{M}$;
		\item \textbf{Budget constraint} the number of coins in $r_{m+1}$ does not exceed the budget; and
		\item \textbf{$\epsilon$-CIK constraint} $r_{m+1}$ is a $\epsilon$-CIK-RS.
	\end{itemize}
\end{definition}

Since the new ring signature should be composed of some modules and modules are disjoint, we can transform the input of the related ring signature $\mathbb{R}$ and the mixins universe $\mathbb{C}$ as the module set $\mathbb{M}$. This procedure is simple and can be done in polynomial time. 

\subsection{The Disjoint-superset Related Ring Signature Set}
\label{subsec: DS-RS}

We first formally define the super ring signature.
\begin{definition}
	(The super ring signature) Given a related ring signature set, $\mathbb{R}_{m}$, a ring signature $r_i \in \mathbb{R}_m$ is a super ring signature if $\forall j \in (i, m],$ $r_i \cap r_j = \emptyset$ and $\forall j \in [1, i)$, if $r_j \cap r_i \neq \emptyset, r_j \subset r_i$. 
\end{definition}

Some ring signatures are the superset of its previous ring signatures. A ring signature is a super ring signature if each its subsequent ring signature is disjoint with it. Here is an example. 

\begin{example}
	There are four ring signatures, $r_1 = \{c_1, c_2\}$, $r_2 = \{c_1, c_2, c_3\}$, $r_3 = \{c_1, c_2, c_3\}$, and $r_4 = \{c_4, c_5\}$. Then, $r_3$ and $r_4$ are two super ring signatures, but $r_1$ and $r_2$ are not.
\end{example}

\begin{definition}
	(The disjoint-superset related ring signature set). A related ring signature set, $\mathbb{R}_{m}$, is a disjoint-superset related ring signature set if, for any two super ring signatures in $\mathbb{R}_m$, they are disjoint.
\end{definition}

The $\mathbb{R}_3$ in Example~\ref{ex:PT} is a disjoint-superset related ring signature set, but the $\mathbb{R}_2$ in Example~\ref{ex:CIA-MS} is not a disjoint-superset related ring signature set, since $r_1 \cap r_2 = c_1$.

%and $Pr_3(c_3, r_2)$ is the same as $Pr_2(c_3,r_2)$. Based on this observation, we prove some significant properties of DS-RSSs.
\subsection{The module}
In this subsection, we formally define the concept of the module.

\begin{definition}
	(The module) A module, denoted by $m_i = \{ns_i, d_i$, $str_i$, $ST_i$, $dive_i, pr_{min}^i, pr_{max}^i\}$, is a super ring signature or a coin that has not been contained in any ring signature, where:
	\begin{itemize}[leftmargin=*]
		\item $ns_i$ is the number of ring signatures which are $r_i$'s subsets in $\mathbb{R}_m$;
		\item $str_i$ is the set of coins which are contained in $srs_i$;
		\item $d_i = |str_i| - ns_i$, namely $srs_i$'s degree;
		\item $ST_i$ is the set of transactions of which a coin in $str_i$ is an output;
		\item $dive_i = |ST_i|$, namely $srs_i$'s diversity;
		\item $pr_{max}^i = \max \{Pr_{m}(c)| c \in str_i\}$; and 
		\item $pr_{min}^i = \min \{Pr_{m}(c)| c \in str_i\}$.
	\end{itemize}
\end{definition}

Specifically, when a module $m_i$ is a coin that has not been contained in any ring signature, $ns_i = 0$, $d_i = 1$, $dive_i = 1$, and $pr_{max}^i = pr_{min}^i =0$. For simplicity, we denote the size of a module $m_i$ is the number of coins in $str_i$, i.e., $|m_i| = |str_i|$.

\subsection{Properties}

When a related ring signature set is a disjoint-superset related ring signature set, there are some significant properties, which can help to retrieve the module set (Theorem ~\ref{theorem:pr(r,a)01},~\ref{theorem:pr_m(r_m,a)01} and~\ref{theorem:pr(a)01}) and reduce the time complexity of verifying if a ring signature is a $\epsilon$-CIK-RS (Theorem~\ref{theorem:pr(a)dandiao},~\ref{theorem:Pr(|)daoPr(c)} and ~\ref{theorem:epsin}). 

We first prove in Theorem~\ref{theorem:pr(r,a)01} that when a related ring signature set is a disjoint-superset related ring signature set, the probability of coin $c$ being spent in the ring signature $r$ will keep stable. 

\begin{theorem}
	\label{theorem:pr(r,a)01}
	Given a disjoint-superset related ring signature set, $\mathbb{R}_m = \{r_1, r_2, \cdots, r_m\}$, we have $\forall i\in [2, m], \forall j <i, \forall c_t \in r_j, Pr_{i}(r_j, c_t) = Pr_{i-1}(r_j, c_t)$
\end{theorem}

\begin{proof}
	According to the Definition~\ref{def:spent coin permutation tree} and ~\ref{def:DS-RRSS}, $\forall i \in [1,m]$, for each node $\kappa$ in $\mathbb{N}_{i, i}$, we can partition $\mathbb{P}_\kappa$ as two sets $\mathbb{P}_\kappa^1$ and $\mathbb{P}_\kappa^2$, where $\mathbb{P}_\kappa^1 \subseteq r_i$, $\mathbb{P}_\kappa^2 \cap r_i = \emptyset$, and $\mathbb{P}_\kappa^1 \cup \mathbb{P}_\kappa^2 = \mathbb{P}_\kappa$. Thus, $|\mathbb{P}_\kappa^1| = ns_i$. Since each ring signature spent an unspent coin, $\forall i \in [2, m]$, $|r_i| > ns_i$. Thus, according to the Definition~\ref{def:spent coin permutation tree}, $\forall i \in [2,m], \forall j < i$, $\mathbb{N}_{i,j} = \mathbb{N}_{i-i,j}$ and for each node $\kappa \in \mathbb{N}_{i, i-1}$, it has $d_i$ children. Thus, $\forall i \in [2,m], \forall j<i, \forall c_t \in r_j, \mathbb{N}_{i,i-1}^{j, t} = \mathbb{N}_{i-1,i-1}^{j,t}$.Therefore, according to the Equation~\ref{eq:pr_f(c,r)}, $\forall i \in [2,m], \forall j < i, \forall c \in r_j$, $Pr_i(r_j, c_t) = \frac{|\mathbb{N}_{i,i}^{j,t}|}{|\mathbb{N}_{i,i}|} = \frac{|\mathbb{N}_{i-1,i-1}^{j,t}| \cdot d_i}{|\mathbb{N}_{i-1,i-1}|\cdot d_i}$ $= \frac{|\mathbb{N}_{i-1,i-1}^{j,t}|}{|\mathbb{N}_{i-1,i-1}|} =Pr_{i-1}(r_j, c_t)$.
\end{proof}

Next, we prove in Theorem~\ref{theorem:pr_m(r_m,a)01} that when a related ring signature set is a disjoint-superset related ring signature set, the probability of a coin $c_t$ being spent in the latest ring signature set, $r_m$, can be calculated iteratively.

\begin{theorem}
	\label{theorem:pr_m(r_m,a)01}
	Given a disjoint-superset related ring signature set $\mathbb{R}_m = \{r_1, r_2, \cdots, r_m\}$, $\forall c_t \in r_m$, we have $Pr_m(r_m, c_t) = \frac{1 - Pr_{m-1}(c_t)}{d_i}$. 
\end{theorem}

\begin{proof}
	As proved in Theorem~\ref{theorem:pr(r,a)01}, each node in $\mathbb{N}_{m, m-1}$ has $d_{m}$ children and $\forall c_t \in r_{m-1}, \mathbb{N}_{m,m-1}^{m-1, t} = \mathbb{N}_{m-1,m-1}^{m-1,t}$. According to the Equation~\ref{eq:pr_f(c,r)}, $\forall c_t \in r_m$, 
	\begin{align*}
	Pr_m(r_m, c_t) &=  \frac{|\mathbb{N}_{m,m}^{m,t}|}{|\mathbb{N}_{m,m}|}  =\frac{|\mathbb{N}_{m,m-1}|-\sum_{j=1}^{m-1}|\mathbb{N}_{m,m-1}^{j,t}|}{|\mathbb{N}_{m,m-1}|\cdot(d_i)} \\ 
	& =\frac{\frac{|\mathbb{N}_{m,m-1}|}{|\mathbb{N}_{m,m-1}|}-\frac{\sum_{j=1}^{m-1}|\mathbb{N}_{m,m-1}^{j,t}|}{|\mathbb{N}_{m,m-1}|}}{d_m} \\
	& = \frac{1- Pr_{m-1}(c_t)}{d_m}.
	\end{align*}
	%$Pr_m(r_m, c_t) = %\frac{|\mathbb{N}_{m,m}^{m,t}|}{|\mathbb{N}_{m,m}|} 
	%=\frac{|\mathbb{N}_{m,m-1}|-\sum_{j=1}^{m-1}|\mathbb{N}_{m,m-1}^{j,t}|}{|\mathbb{N}_{m,m-1}|\cdot(d_i)} \\ 
	%=\frac{\frac{|\mathbb{N}_{m,m-1}|}{|\mathbb{N}_{m,m-1}|}-\frac{\sum_{j=1}^{m-1}|\mathbb{N}_{m,m-1}^{j,t}|}{|\mathbb{N}_{m,m-1}|}}{d_m} = \frac{1- Pr_{m-1}(c_t)}{d_m}$.
\end{proof}

Then, we show %in Theorem~\ref{theorem:pr(a)01} 
that when a related ring signature set is a disjoint-superset related ring signature set, the probability of a coin $c$ having been spent in $\mathbb{R}$ can be calculated iteratively.

\begin{theorem}
	\label{theorem:pr(a)01}
	Given a disjoint-superset related ring signature set, $\mathbb{R}_m$, we have {\scriptsize$\forall i \in [1, m], \forall c$, $
		%\begin{equation*}
		Pr_i(c) =
		\begin{cases}
		Pr_{i-1}(c) & \mbox{$c \notin r_i$} \\
		Pr_{i-1}(c) + \frac{1 - Pr_{i-1}(c)}{d_i} & \mbox{$c \in r_i$} 
		\end{cases},
		%\end{equation*}
		$}
	where $Pr_0(c) = 0$. 
\end{theorem}

\begin{proof}
	As proved, {\scriptsize$\forall i \in [2,m], \forall j < i, \forall c_t \in r_j$, $\mathbb{N}_{i,i-1}^{j, t} = \mathbb{N}_{i-1,i-1}^{j,t}$} and each node in $\mathbb{N}_{i, i-1}$ has $d_i$ children. Thus, $\forall i \in [2,m], \forall c_t \in r_i$, 
	\begin{align*}
	Pr_i(c_t) & = \frac{\sum_{j=1}^{i}|\mathbb{N}_{i,i}^{j,t}|}{|\mathbb{N}_{i,i}|} \\ & =\frac{(|\mathbb{N}_{i,i-1}|-\sum_{j=1}^{i-1}|\mathbb{N}_{i,i-1}^{j,t}|)+d_i\cdot\sum_{j=1}^{i-1}|\mathbb{N}_{i,i-1}^{j,t}|}{|\mathbb{N}_{i-1,i-1}|\cdot d_i} \\
	& = \frac{\sum_{j=1}^{i-1}|\mathbb{N}_{i,i-1}^{j,t}|}{|\mathbb{N}_{i-1,i-1}|}+ \frac{1 - \frac{\sum_{j=1}^{i-1}|\mathbb{N}_{i,i-1}^{j,t}|}{|\mathbb{N}_{i-1,i-1}|}}{d_i}  \\
	& = Pr_{i-1}(c_t) + \frac{1-Pr_{i-1}(c_t)}{d_i}.
	\end{align*}
		%$Pr_i(c_t)$ $= \frac{\sum_{j=1}^{i}|\mathbb{N}_{i,i}^{j,t}|}{|\mathbb{N}_{i,i}|} %=\frac{(|\mathbb{N}_{i,i-1}|-\sum_{j=1}^{i-1}|\mathbb{N}_{i,i-1}^{j,t}|)+(d_i)\cdot\sum_{j=1}^{i-1}|\mathbb{N}_{i,i-1}^{j,t}|}{|\mathbb{N}_{i-1,i-1}|\cdot(d_i)}$
		%= \frac{\sum_{j=1}^{i-1}|\mathbb{N}_{i,i-1}^{j,t}|}{|\mathbb{N}_{i-1,i-1}|}+$ $\frac{1 - \frac{\sum_{j=1}^{i-1}|\mathbb{N}_{i,i-1}^{j,t}|}{|\mathbb{N}_{i-1,i-1}|}}{d_i} 
		%= Pr_{i-1}(c_t) + \frac{1-Pr_{i-1}(c_t)}{d_i}$}. 
		By %Definition~\ref{def:spent coin permutation tree} and
	Equation~\ref{eq:pr_f(c)}, {\small$\forall c \in r_1, Pr_1(c) = \frac{1}{|r_1|}$}. Similarly, we can prove {\small$\forall i \in [1,m], \forall c \notin r_i, Pr_i(c) = Pr_{i-1}(c)$}. 
\end{proof}

Thus, given a disjoint-superset related ring signature set, $\mathbb{R}_m$, we can easily retrieve the corresponding module set $\mathbb{M}$. Besides, for any two coins $c, c'$ in the same ring signature $r_i$, we proved that if $Pr_i(c) \leq Pr_i(c')$, $\forall j \geq i, Pr_j(c) \leq Pr_j(c')$.

\begin{theorem}
	\label{theorem:pr(a)dandiao}
	Given a disjoint-superset related ring signature set, $\mathbb{R}_m$, $\forall i \in [1, m], \forall j \leq i, \forall c, c' \in r_j$, if $Pr_j(c) \leq Pr_j(c')$, it holds that $Pr_{i}(c) \leq Pr_{i}(c')$.
\end{theorem}
\begin{proof}
	By Definition~\ref{def:DS-RRSS}, $\forall i \in [1,m], \forall j \leq i, \forall c, c' \in r_j$, if $c \in r_i$, $c' \in r_i$. Thus,
	\begin{align*}
	& Pr_{i+1}(c) - Pr_{i+1}(c') \notag \\
	= & Pr_{i}(c)+\frac{1-Pr_i(c)}{d_i} - Pr_{i}(c') - \frac{1-Pr_i(c')}{d_i} \notag \\
	= & [Pr_{i}(c)- Pr_i(c')] - \frac{1}{d_i} \cdot [Pr_i(c) - Pr_i(c')]
	\end{align*}
	%{\scriptsize$
	%	Pr_{i+1}(c) - Pr_{i+1}(c') 
	%	= Pr_{i}(c)+\frac{1-Pr_i(c)}{d_i} - Pr_{i}(c') - \frac{1-Pr_i(c')}{d_i}$}
	%$=  [Pr_{i}(c)- Pr_i(c')] - \frac{1}{d_i} \cdot [Pr_i(c) - Pr_i(c')].
	%$
	Since $d_i \geq 1$ and $Pr_i(c) \leq Pr_i(c')$, {\scriptsize$Pr_{i+1}(c) - Pr_{i+1}(c') \leq 0$}.
\end{proof}

Furthermore, for any two coins $c, c'$ in the same ring signature $r_j$, we proved that if $Pr_i(r_j|c) \leq Pr_i(r_j|c')$, $\forall k \in[j-1,i], Pr_k(c) \geq Pr_k(c')$.

\begin{theorem}
	\label{theorem:Pr(|)daoPr(c)}
	Given a disjoint-superset related ring signature set, $\mathbb{R}_m$, $\forall i \in [1, m], \forall j \leq i, \forall c, c' \in r_j$, if $Pr_i(r_j|c) \leq Pr_i(r_j|c')$, $\forall k \in [j-1,i], Pr_{k}(c) \geq Pr_{k}(c')$. 
\end{theorem}

\begin{proof}
	Denote $F(t,j,i)$ as a function to recursively calculate $Pr_i(c_t)$ from $Pr_j(c_t)$. As proved in Theorem~\ref{theorem:pr(a)dandiao}, $F(t,j,i)$ increases when $Pr_{j}(c_t)$ increases. 
	By Definition~\ref{def:DS-RRSS}, $\forall i \in [1,m], \forall j \leq i, \forall c, c' \in r_j$,  if $c \in r_i$, $c' \in r_i$. %According to Theorem~\ref{theorem:pr(a)01}, $\forall i \in  [1, m], \forall c \in \mathbb{C}$, we can calculate $Pr_i(c)$ recursively. Suppose $F_{j \rightarrow i}(c)$ is a function 
	By Theorem~\ref{theorem:pr(r,a)01} and ~\ref{theorem:pr(a)01}, $\forall i \in [2, m], \forall j\leq i, \forall c_t \in r_j$, $Pr_i(r_j|c_t) = \frac{Pr_i(r_j, c_t)}{Pr_i(c_t)} = \frac{Pr_j(r_j,c_t)}{F_{i \leftarrow j-1}(c_t)} = \frac{\frac{1-Pr_{j-1}(c_t)}{d_j}}{F(t,j-1,i)}$. Thus, $Pr_i(r_j|c_t)$ increases when $Pr_{j-1}(c_t)$ decreases.
	Thus, $\forall i \in [1, m], \forall j \leq i, \forall c, c' \in r_j$, if $Pr_i(r_j|c) \leq Pr_i(r_j|c')$, $Pr_{j-1}(c) \geq Pr_{j-1}(c')$. Then by Theorem~\ref{theorem:pr(a)dandiao}, we have $\forall i \in [1, m], \forall j \leq i, \forall c, c' \in r_j$, $\forall k \in [j-1,i], Pr_{k}(c) \geq Pr_{k}(c')$.
\end{proof}

Then we prove that, if the conditional probabilities $Pr_{i}(r_j|c_t)$ of two coins in a ring signature satisfy $\epsilon$-CI, the conditional probabilities of these two coins in subsequent ring signatures also satisfy $\epsilon$-CI.

\begin{theorem}
	\label{theorem:epsin}
	Given a disjoint-superset related ring signature set, $\mathbb{R}_m$, $\forall i \in [1, m], \forall j \leq i, \forall c, c' \in r_j$, if {\small$Pr_i(r_j|c) \geq Pr_i(r_j|c')$} and $\frac{Pr_i(r_j|c)}{Pr_i(r_j|c')} = \beta$, it holds that {\small$\forall k \in (i,m] \land r_i \subseteq r_k, Pr_{k}(r_j|c) \geq Pr_{k}(r_j|c')$} and $\frac{Pr_k(r_j|c)}{Pr_k(r_j|c')} = \beta'\leq\beta$. 
\end{theorem}
\begin{proof}
	By Theorem~\ref{theorem:Pr(|)daoPr(c)}, if $Pr_i(r_j|c) \geq Pr_i(r_j|c')$, $Pr_i(c) \leq Pr_i(c')$. Furthermore, by Theorem~\ref{theorem:pr(a)dandiao}, $\forall k \in [i-1,m] \land r_i \subseteq r_k$, $Pr_k(c) \leq Pr_i(c')$ and $Pr_{i+1}(r_j|c) \geq Pr_{i+1}(r_j|c')$. %If $\frac{Pr_i(r_j|c)}{Pr_i(r_j|c')} = \beta$, we have $\frac{Pr_i(r_j,c)}{Pr_i(r_j,c')} \cdot \frac{Pr_i(c')}{Pr_i(c)} = \beta$.
	Then, by Theorem~\ref{theorem:pr(r,a)01} and ~\ref{theorem:pr(a)01}, $ 
	\beta' = \frac{Pr_{i+1}(r_j|c)}{Pr_{i+1}(r_j|c')}
	= \frac{Pr_i(r_j,c)}{Pr_i(c) + \frac{1-Pr_i(c)}{d_i}} \cdot \frac{Pr_i(c') + \frac{1-Pr_i(c')}{d_i}}{Pr_i(r_j,c')}
	=  \frac{Pr_i(r_j,c)}{Pr_i(r_j,c')} \cdot \frac{(d_i-1)Pr_i(c')+1}{(d_i-1)Pr_i(c)+1}$. 
	When $d_i-1 \geq 1$, $\beta' \leq \frac{Pr_i(r_j,c)}{Pr_i(r_j,c')} \cdot \frac{Pr_i(c')}{Pr_i(c)} = \beta$. When $d_i-1 =0$, since $\frac{Pr_i(c')}{Pr_i(c)} \geq 1$, $\beta' = \frac{Pr_i(r_j,c)}{Pr_i(r_j,c')} \leq \frac{Pr_i(r_j,c)}{Pr_i(r_j,c')} \cdot \frac{Pr_i(c')}{Pr_i(c)} = \beta$.
\end{proof}

Thus, if the new ring signature is the superset of some modules in $\mathbb{M}$ and it satisfy $\epsilon$-CI, it is a $\epsilon$-CIK-RS. In other words, to verify if a new ring signature is a $\epsilon$-CIK-RS, we just need to verify if it satisfy $\epsilon$-CI, which decreases the time complexity form $\mathcal{O}(\sum_{i=1}^{|\mathbb{R}|+1}|r_i|^2)$ to $\mathcal{O}(|r_{m+1}|^2)$. Besides, suppose $pr_{max} = \max \{pr_m(c)| c \in r_{m+1}\}$ and $pr_{min} = \min \{pr_m(c)| c \in r_{m+1} \}$. And according to  Definition~\ref{def:CI}, Theorem~\ref{theorem:pr(a)01} and Theorem~\ref{theorem:pr_m(r_m,a)01}, to verify if $r_{m+1}$ satisfy $\epsilon$-CI, we just need to verify if $\frac{(1-pr_{max})\cdot e^\epsilon}{(d_{m+1}-1)\cdot pr_{max}+1} \geq \frac{(1-pr_{min})}{(d_{m+1}-1)\cdot pr_{min}+1}$, which further decreases the time complexity from $\mathcal{O}(|r_{m+1}|^2)$ to $\mathcal{O}(|r_{m+1}|)$. 

%And the mixin universe $\mathbb{C}$ can be represented by the union of the SRS set $\mathbb{SRS}$ and the fresh coin set $\mathbb{F}$.

\subsection{Hardness of CIA-MS-DS}
In this subsection, we prove that the CIA-MS-DS problem is NP-hard by reducing 0-1 knapsack problem~\cite{2013approximation}.

\begin{theorem}
	\label{theorem:np}
	%(Hardness of CIA-MS-DS problem) 
	The CIA-MS-DS problem is NP-hard.
\end{theorem}

\begin{proof}
	We prove the theorem by a reduction from the 0-1 knapsack problem~\cite{2013approximation}, which can be described as follows: Given a set, $I$, of $n$ items $i$ numbered from 1 up to $n$, each with a weight $w_i$ and a value $x_i$, along with a maximum weight capacity $C$, the 0-1 knapsack problem is to find a subset $I'$ of $I$ that maximizes $\sum_{i \in I'}x_i$ subjected to $\sum_{c_j \in r_k} w_i \leq C$.
	
	For a given 0-1 knapsack problem instance, we can transform it into a special CIA-MS-DS problem instance as follows: we generate a module set, $\mathbb{M}$, where there are $n$ modules numbered from 1 up to $n$, each with a size $x_i$ and diversity $w_i$. The $\epsilon$ is large enough that any combination of modules in $\mathbb{M}$ is a $\epsilon$-CIK-RS. And for any two modules, their source transaction sets are disjoint. Thus, $dive_{r_{m+1}} = \sum_{m_i \in r_{m+1}} dive_{i}$.
	
	Thus, to find the new ring signature $r_{m+1}$ whose diversity is maximum is equal to find a maximum assignment of 0-1 knapsack problem. Given this mapping, we can reduce the 0-1 knapsack problem to the CIA-MS-DS problem. Since the 0-1 knapsack problem is known to be NP-hard~\cite{2013approximation}, the CIA-MS-DS problem is also NP-hard.
\end{proof}
